Deep Gaussian Processes for Multi-fidelity Modeling

Multi-fidelity methods are prominently used when cheaply-obtained, but possibly biased and noisy, observations must be effectively combined with limited or expensive true data in order to construct reliable models. This arises in both fundamental machine learning procedures such as Bayesian optimization, as well as more practical science and engineering applications. In this paper we develop a novel multi-fidelity model which treats layers of a deep Gaussian process as fidelity levels, and uses a variational inference scheme to propagate uncertainty across them. This allows for capturing nonlinear correlations between fidelities with lower risk of overfitting than existing methods exploiting compositional structure, which are conversely burdened by structural assumptions and constraints. We show that the proposed approach makes substantial improvements in quantifying and propagating uncertainty in multi-fidelity set-ups, which in turn improves their effectiveness in decision making pipelines.

==> figures/dgp_mf_arch_3l.tex <==
\begin{tikzpicture}

		\node[latent]  (FL) 	{{$ \hphantom{a}\fvect_3^{\textcolor{red!40!gray}{\textbf{3}}}$\hphantom{b}}};
		\node[latent, left=2 of FL]  (F2) 		{{$ \hphantom{a}\fvect_2^{\textcolor{blue!40!gray}{\textbf{2}},\textcolor{red!40!gray}{\textbf{3}}}$}};
		\node[latent, left=2 of F2]  (F1) 		{{$\fvect^{\textcolor{green!40!gray}{\textbf{1}},\textcolor{blue!40!gray}{\textbf{2}},\textcolor{red!40!gray}{\textbf{3}}}_1$}};
		
		\node[obs, above=.8 of F1]		(X1) 	{$\textbf{X}^{\textcolor{green!40!gray}{\textbf{1}},\textcolor{blue!40!gray}{\textbf{2}},\textcolor{red!40!gray}{\textbf{3}}}$};
		\node[obs, above=.8 of F2]		(X2) 	{$\hphantom{a}\textbf{X}^{\textcolor{blue!40!gray}{\textbf{2}},\textcolor{red!40!gray}{\textbf{3}}}$};
		\node[obs, above=.8 of FL]		(XL) 	{$\hphantom{a}\textbf{X}^{\textcolor{red!40!gray}{\textbf{3}}}\hphantom{b}$};
		
		\node[obs, below=.8 of F1]		(y1) 	{$\textcolor{green!40!gray}{\textbf{y}^\textbf{1}}$};
		\node[obs, below=.8 of F2]		(y2) 	{$\textcolor{blue!40!gray}{\textbf{y}^\textbf{2}}$};
		\node[obs, below=.8 of FL] 		(yL)	{$\textcolor{red!40!gray}{\textbf{y}^\textbf{3}}$};
		
%		\edge[->] {X2} {F2};
%		\edge[->] {XL} {FL};
		
		\edge[->] {F1} {y1} ;
		\edge[->] {F2} {y2} ;
		\edge[->] {FL} {yL} ;
		
		\edge[->] {F1} {F2} ;
		\edge[->] {F2} {FL} ;
		
		\edge[->] {X1}{F1}
		\edge[->] {X2}{F2}
		\edge[->] {XL}{FL}
		
\end{tikzpicture}
\vspace{.3cm}

==> figures/dgp_mf_pred_3l.tex <==
\begin{tikzpicture}

		\node[latent]  (FL) 	{{$f_3^{\star}$}};
		\node[latent, left=2 of FL]  (F2) 	{{$f_2^{\star}$}};
		\node[latent, left=2 of F2]  (F1) 	{{$f_1^{\star}$}};
		
		\node[obs, above=.8 of F1]		(X1) {{$\textbf{x}^{\star}$}};
		\node[obs, above=.8 of F2]		(X2) {{$\textbf{x}^{\star}$}};
		\node[obs, above=.8 of FL]		(XL) {{$\textbf{x}^{\star}$}};
		
		\node[below=.8 of F1]		(y1) 	{${y}_1^\star$};
		\node[below=.8 of F2]		(y2) 	{${y}_2^\star$};
		\node[below=.8 of FL] 		(yL)	{${y}_3^\star$};
		
%		\edge[->] {X2} {F2};
%		\edge[->] {XL} {FL};
		
		\edge[->] {F1} {y1} ;
		\edge[->] {F2} {y2} ;
		\edge[->] {FL} {yL} ;
		
		\edge[->] {F1} {F2} ;
		\edge[->] {F2} {FL} ;
		
		\edge[->] {X1}{F1}
		\edge[->] {X2}{F2}
		\edge[->] {XL}{FL}
		
\end{tikzpicture}
\vspace{.3cm}

==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

